Stochastic Answer Networks for Natural Language Inference

We propose a stochastic answer network (SAN) to explore multi-step inference strategies in Natural Language Inference. Rather than directly predicting the results given the inputs, the model maintains a state and iteratively refines its predictions. Our experiments show that SAN achieves the state-of-the-art results on three benchmarks: Stanford Natural Language Inference (SNLI) dataset, MultiGenre Natural Language Inference (MultiNLI) dataset and Quora Question Pairs dataset.

==> Natural Language Inference/experiments.tex <==
\section{Experiments}
\label{sec:exp}
%\vspace{-0.2cm}
\subsection{Dataset}
\label{sec:data}
Here, we evaluate our model in terms of accuracy on four benchmark datasets. \textbf{SNLI} \cite{bowman2015large} contains 570k human annotated sentence pairs, in which the premises are drawn from the captions of the Flickr30 corpus, and hypothesis are manually annotated. \textbf{MultiNLI} \cite{2017arXiv170405426W} contains 433k sentence pairs, which are collected similarly as SNLI. However, the premises are collected from a broad range of genre of American English. The test and development sets are further divided into in-domain (\textbf{matched}) and cross-domain (\textbf{mismatched}) sets.  %For both datasets, it has three types of relation\footnote{In SNLI, the label ``-" denotes inconsistency between annotators, and it is removed during the training and test.}%: \textit{entailment}, \textit{neutral} and \textit{contradiction}.
The Quora Question Pairs dataset \cite{wang2017bilateral} is proposed for paraphrase identification. It contains 400k question pairs, and each question pair is annotated with a binary value indicating whether the two questions are paraphrase of each other. %Note that we use the standard data splits for training, development and test.
\textbf{SciTail} dataset is created from a science question answering (SciQ) dataset. It contains 1,834 questions with 10,101 \textit{entailments} examples and 16,925 \textit{neutral} examples. Note that it only contains two types of labels, so is a binary task. 
%\textcolor{blue}{\textbf{SciTail} dataset is created for Science question answering task. It is from publicly released 4th grad (204 questions) and 8th grade (195 questions) exams and 2,835 crowed-sourced questions.} 
\subsection{Implementation details}
\label{sec:imp}
The spaCy tool\footnote{https://spacy.io} is used to tokenize all the dataset and PyTorch is used to implement our models. We fix word embedding with 300-dimensional GloVe word vectors \cite{pennington2014glove}. For the character encoding, we use a concatenation of the multi-filter Convolutional Neural Nets with windows $1, 3, 5$ and the hidden size $50, 100, 150$.\footnote{We limit the maximum length of a word by 20 characters. The character embedding size is set to 20.} So lexicon embeddings are $d$=600-dimensions. The embedding for the out-of-vocabulary is zeroed. The hidden size of LSTM in the contextual encoding layer, memory generation layer is set to 128, thus the input size of output layer is 1024 (128 * 2 * 4) as Eq~\ref{eq:begin}. The projection size in the attention layer is set to 256. To speed up training, we use weight normalization \cite{salimans2016weight}. The dropout rate is 0.2, and the dropout mask is fixed through time steps \cite{gal2016theoretically} in LSTM. The mini-batch size is set to 32. Our optimizer is Adamax \cite{kingma2014adam} and its learning rate is initialized as 0.002 and decreased by 0.5 after each 10 epochs.
%%%%%%%%%%%%Multi-hop%%%%%%%%%%%%
%\begin{table}[t!]
%\centering
%\begin{tabular}{@{\hskip1pt}l || c | c  }
%\hline
%%\multicolumn{3}{c}{ Model Comparison (Accuracy)} \\ \hline
%\multirow{2}{*}{Model}& \multicolumn{2}{c}{MultiNLI Dev (Accuracy\%)} \\ \cline{2-3}
%&\multicolumn{1}{ c| }{Matched}& Mismatched   \\ \hline
%Single-step & 78.69 & 78.83\\ \hline
%%Fixed 5-step &78.54 &79.21 \\ \hline
%MIN & \textbf{79.88} & \textbf{79.91} \\ \hline \hline
%&\multicolumn{2}{c}{ SNLI Dev (Accuracy\%)} \\ \hline \hline
%%&Dev & Test \\ \hline
%Single-step & \multicolumn{2}{c} {88.32}\\ \hline
%%Fixed 5-step &88.40 & 88.03 \\ \hline
%MIN &\multicolumn{2}{c}{\textbf{88.73}} \\ \hline \hline
%&\multicolumn{2}{c}{ Quora Question Dev (Accuracy\%)} \\ \hline \hline
%%&Dev & Test \\ \hline
%Single-step &\multicolumn{2}{c}{ 89.67}\\ \hline
%%Fixed 5-step &89.61 & 88.78 \\ \hline
%MIN & \multicolumn{2}{c}{\textbf{89.70}}\\ \hline
%\end{tabular}
%\caption{\label{tab:main} Comparison of different inference strategies on MultiNLI, SNLI and Quora Question datasets.}
%\end{table}


\begin{table}[t!]
\centering
\begin{tabular}{@{\hskip1pt}l || c | c  }
\hline
 & Single-step & SAN \\\hline
MultiNLI matched & 78.69 & \textbf{79.88} \\
MultiNLI mismatched & 78.83 & \textbf{79.91} \\ \hline 
%MultiNLI matched & 78.69 & \textbf{79.88} \\
%MultiNLI mismatched & 78.83 & \textbf{79.91} \\ \hline 
SNLI & 88.32 & \textbf{88.73} \\ \hline
Quora & 89.67 & \textbf{90.70} \\ \hline
SciTail &85.46  & \textbf{89.35} \\ \hline
% JOCI-A &\textbf{1.83} & 1.89  \\ 
% JOCI-B &\textbf{1.95} & 1.97 \\ \hline
\end{tabular}
\caption{\label{tab:main} Comparison of single and multi-step inference strategies on MultiNLI, SNLI, Quora Question and SciTail \textbf{dev} sets.}
\end{table}

%%%% Backup table 1
% \begin{table}[t!]
% \centering
% \begin{tabular}{@{\hskip1pt}l || c | c  }
% \hline
% %\multicolumn{3}{c}{ Model Comparison (Accuracy)} \\ \hline
% \multirow{2}{*}{Model}& \multicolumn{2}{c}{MultiNLI Dev (Accuracy\%)} \\ \cline{2-3}
% &\multicolumn{1}{ c| }{Matched}& Mismatched   \\ \hline
% Single-step & 78.69 & 78.83\\ \hline
% %Fixed 5-step &78.54 &79.21 \\ \hline
% MIN & \textbf{79.88} & \textbf{79.91} \\ \hline \hline
% \multicolumn{3}{c}{ SNLI Dataset (Accuracy\%)} \\ \hline \hline
% &Dev & Test \\ \hline
% Single-step & 88.32 & 87.89\\ \hline
% %Fixed 5-step &88.40 & 88.03 \\ \hline
% MIN & \textbf{88.73} & \textbf{88.51} \\ \hline \hline
% \multicolumn{3}{c}{ Quora Question Dataset (Accuracy\%)} \\ \hline \hline
% %&Dev & Test \\ \hline
% Single-step & 89.67 & 88.96\\ \hline
% %Fixed 5-step &89.61 & 88.78 \\ \hline
% MIN & \textbf{89.70} & \textbf{89.39} \\ \hline
% \end{tabular}
% \caption{\label{tab:main} Comparison of different inference strategies on MultiNLI, SNLI and Quora Question datasets.}
% \end{table}

\subsection{Results}
\label{sec:result}
%\subsection{Main results}
One main question which we would like to address is whether the multi-step inference help on NLI. 
We fixed the lower layer and only compare different architectures for the output layer:%\vspace{-0.2cm}
\begin{enumerate}
\item \textit{Single-step}: Predict the relation using Eq~\ref{eq:begin} based on $s_0$ and $x_0$. Here, $x_0=\sum_j \alpha_j M^p_{j}$, where $\alpha_j = \frac{exp(w \cdot M^p_j)}{\sum_{j'}exp(w \cdot M^p_{j'})}$\footnote{For direct comparison, this has the same three lower layers as Fig. \ref{fig:model} and only changes the answer module.}.
\item \textit{SAN}: The multi-step inference model. We use 5-steps with the prediction dropout rate $0.2$ on the all experiments.
\end{enumerate} 

%For experiments on MultiNLI dataset, we select the model based on the total sum of accuracy on both the matched development dataset and mismatched development dataset. However, for SNLI and Quora Question datasets, we select model only based on development dataset.
%Table~\ref{tab:main} shows that our model outperforms both the single-step and the fixed 5-step models and, achieves best on MultiNLI and SNLI, e.g., 79.88 (vs single-step: 78.69 and fixed 5-step: 78.54) and 79.91 (vs single-step: 78.83 and fixed 5-step: 79.21) on MultiNLI matched and mismatched development dataset, respectively.
%{\color{red}Question for Xiaodong: I couldn't figure out how these numbers match up with which cell in Table 2. Further, I would take out the fixed 5-step model vs SAN/MIN comparison and just focussed on single-step vs MIN, as follows:}

Table~\ref{tab:main} shows that our multi-step model consistently outperforms the single-step model on the dev set of all four datasets in terms of accuracy. For example, %on MultNLI matched condition, SAN achieves 79.88 while single-step achieves 78.69 . 
on SciTail dataset, SAN outperforms the single-step model by +3.89 (85.46 vs 89.35). 

We compare our results with the state-of-the-art in Table~\ref{tab:comp}. Our model achieves the best performance on SciTai and Quora Question tasks. For instance, SAN obtains 89.4 (vs 89.1) and 88.4 (88.3) on the Quora Question and SciTail test set, respectively and set the new state-of-the-art. On SNLI and MultiNLI dataset, ESIM+ELMo \cite{peters2018deep}, GPT \cite{radford2018improving} and BERT \cite{devlin2018bert} use a large amount of external knowledge or a large scale pretrained contextual embeddings. However, SAN is still competitive these models. On SciTail dataset, SAN even outperforms GPT.  
Due to the space limitation, we only list two top models.\footnote{See leaderboard for more information: https://www.kaggle.com/c/multinli-matched-open-evaluation, https//www.kaggle.com/c/multinli-mismatched-open-evaluation, https://nlp.stanford.edu/projects/snli, http://data.allenai.org/scitail/leaderboard/.}

We further utilize BERT as a feature extractor\footnote{We run BERT (the base model) to extract embeddings of both premise and hypothesis and then feed it to answer models for a fair comparison.} and use the SAN answer module on top of it. Comparing with \textit{Single-step} baseline, the proposed model obtains +2.8 improvement on the SciTail test set (94.0 vs 91.2) and +2.1 improvement on the SciTail dev set (96.1 vs 93.9). This shows the generalization of the proposed model which can be easily adapted on other models \footnote{Due to highly time consumption and space limitation, we omit the results using BERT on SNLI/MNLI/Quora Question dataset.}.

%Furthermore, with the help of ELMo, our model achieves the state-of-the-art.
%Due to the space limitation, we only list two top models (ref: MultiNLI\footnote{https://www.kaggle.com/c/multinli-matched-open-evaluation}$^,$\footnote{https//www.kaggle.com/c/multinli-mismatched-open-evaluation}, SNLI\footnote{https://nlp.stanford.edu/projects/snli}, Quora Question Pairs \cite{2017arXiv170904348G} and SciTail\footnote{http://data.allenai.org/scitail/leaderboard/} for more information.)

%%%%%%%%%%%Leadboard%%%%%%%%%%%%%
%\begin{table}[t!]
%\centering
%\begin{tabular}{@{\hskip1pt}l @{\hskip1pt}||@{\hskip1pt} c |@{\hskip1pt} c  @{\hskip1pt}}
%\hline
%\multirow{2}{*}{Model}& \multicolumn{2}{c}{MultiNLI Test} \\ \cline{2-3}
%&\multicolumn{1}{ @{\hskip1pt} c| @{\hskip1pt}}{Matched}& Mismatched   \\ \hline
%DIIN\cite{2017arXiv170904348G} & 78.8 & 77.8\\ \hline
%CAFE\cite{2018arXiv180100102T} & 78.7 & 77.9 \\ \hline
%MIN & \textbf{79.3} & \textbf{78.7} \\ \hline \hline
%Ensemble &Matched & Mismatched \\ \hline
%DIIN\cite{2017arXiv170904348G} & 80.0 & 78.7 \\ \hline
%CAFE\cite{2018arXiv180100102T} & 80.2 & 79.0 \\ \hline
%MIN* & \textbf{80.6} & \textbf{80.1} \\ \hline \hline
%\multicolumn{3}{c}{ SNLI Dataset (Accuracy\%)} \\ \hline
%&Train & Test \\ \hline
%CAFE\cite{2018arXiv180100102T} &89.8 &88.5\\ \hline
%KIM\cite{2017arXiv171104289C} &94.1 &\textbf{88.6}\\ \hline
%MIN & \textbf{94.6} & \textbf{88.5} \\ \hline \hline
%\multicolumn{3}{c}{ Quora Question Dataset (Accuracy\%)} \\ \hline \hline
%&Dev & Test \\ \hline
%DecAtt\cite{tomar2017neural} & 88.9 & 88.4\\ \hline
%DIIN\cite{2017arXiv170904348G} &89.4 & 89.1 \\ \hline
%MIN & \textbf{89.7} & \textbf{89.4} \\ \hline
%\end{tabular}
%\caption{\label{tab:comp} Comparison with the state-of-the-art on MultiNLI, SNLI and Quora Question datasets. *We ensemble three models trained with three different initialization seeds.}
%\end{table}

\begin{table}[t!]
\centering
\begin{tabular}{@{\hskip1pt}l @{\hskip1pt}||@{\hskip1pt} c |@{\hskip1pt} c  @{\hskip1pt}}
\hline
\multirow{2}{*}{Model}& \multicolumn{2}{c}{MultiNLI Test} \\ \cline{2-3}
&\multicolumn{1}{ @{\hskip1pt} c| @{\hskip1pt}}{Matched}& Mismatched   \\ \hline
DIIN\cite{2017arXiv170904348G} & 78.8 & 77.8\\ \hline
%CAFE\cite{2018arXiv180100102T} & 78.7 & 77.9 \\ \hline
BERT\cite{devlin2018bert} & \textbf{86.7} & \textbf{85.9} \\ \hline
{\MIN} & 79.3 & 78.7 \\ \hline \hline
%Ensemble &Matched & Mismatched \\ \hline
%DIIN\cite{2017arXiv170904348G} & 80.0 & 78.7 \\ \hline
%CAFE\cite{2018arXiv180100102T} & 80.2 & 79.0 \\ \hline
%{\MIN}* & \textbf{80.6} & \textbf{80.1} \\ \hline \hline
\multicolumn{3}{c}{ SNLI Dataset (Accuracy\%)} \\ \hline
%CAFE\cite{2018arXiv180100102T} &\multicolumn{2}{c}{88.5}\\ \hline
%KIM\cite{2017arXiv171104289C} &\multicolumn{2}{c}{88.6}\\ \hline
ESIM+ELMo &\multicolumn{2}{c}{88.7} \\ \hline
GPT\cite{radford2018improving} & \multicolumn{2}{c}{\textbf{89.9}}\\ \hline
{\MIN} & \multicolumn{2}{c}{\textbf{88.7}} \\ \hline
%{\MIN} + ELMo & \multicolumn{2}{c}{\textbf{88.8}} \\ \hline
\hline
\multicolumn{3}{c}{ Quora Question Dataset (Accuracy\%)} \\ \hline \hline
%DecAtt\cite{tomar2017neural} &  \multicolumn{2}{c}{88.4}\\ \hline
\cite{tomar2017neural} &  \multicolumn{2}{c}{88.4}\\ \hline
%DIIN\cite{2017arXiv170904348G} &  \multicolumn{2}{c}{ 89.1} \\ \hline
\cite{2017arXiv170904348G} &  \multicolumn{2}{c}{ 89.1} \\ \hline
{\MIN} &  \multicolumn{2}{c}{\textbf{89.4}} \\ \hline
\multicolumn{3}{c}{ SciTail Dataset (Accuracy\%)} \\ \hline \hline
%CompAtt\cite{parikh2016decomposable}  & \multicolumn{2}{c}{ 72.3}\\ \hline
%\cite{parikh2016decomposable}  & \multicolumn{2}{c}{ 72.3}\\ \hline
%DGEM \cite{scitail} &  \multicolumn{2}{c}{ 77.3} \\ \hline
\cite{scitail} &  \multicolumn{2}{c}{ 77.3} \\ \hline
GPT\cite{radford2018improving} & \multicolumn{2}{c}{88.3}\\ \hline
{\MIN} &  \multicolumn{2}{c}{\textbf{88.4}} \\ \hline

%{\MIN} &  \multicolumn{2}{c}{\textbf{80.9}} \\ \hline

% \multicolumn{3}{c}{ JOCI Dataset (MSE) } \\ \hline \hline
% %\multirow{2}{*}{}& \multicolumn{2}{c}{JOCI Dataset (MSE)} \\ \cline{2-3}
% &JOCI--A & JOCI--B \\ \hline
% DGEM \cite{scitail} & \textbf{1.96} & 2.74\\ \hline
% {\MIN} &  1.97& \textbf{2.04}\\ \hline

\end{tabular}
\caption{\label{tab:comp} Comparison with the state-of-the-art on MultiNLI, SNLI and Quora Question \textbf{test} sets.}% *We ensemble three models trained with three different initialization seeds.}
\end{table}

\begin{table}[ht!]
\centering
\begin{tabular}{@{\hskip1pt}l |@{\hskip1pt} l |@{\hskip1pt} c |@{\hskip1pt} c | c }
\hline
\multirow{2}{*}{Tag}& \multicolumn{2}{c|@{\hskip1pt}}{Matched}& \multicolumn{2}{c}{Mismatched} \\ \cline{2-5}
&Chen$^1$& {\MIN} & Chen$^1$& {\MIN} \\ \hline  \hline
Conditional &\textbf{100\%}  &65\%	&\textbf{100\%} &81\%\\ \hline 
Word overlap	&63 \% &\textbf{86\%} &76\% &\textbf{92\%}\\ \hline
Negation &75\%  &\textbf{80\%} &72\% &\textbf{79\%}\\ \hline
Antonym &50\% &\textbf{77\%} &58\% &\textbf{85\%}	\\ \hline 
Long Sentence	&67\% &\textbf{84\%} &67\% &\textbf{79\%}\\ \hline 
Tense Difference &\textbf{86\%}	 &75\% &\textbf{89\%} &83\%\\ \hline 
Active/Passive &88\%	&\textbf{100\%} &91\% &\textbf{100\%}\\ \hline 
Paraphrase&78\% &\textbf{92\%} &89\% &\textbf{92\%} \\\hline 
Quantity/Time&33\%	  &\textbf{53\%}& 46\% &\textbf{51\%} \\ \hline 
Coreference	 &\textbf{83\%}	 & 73\% &80\% &\textbf{84\%}\\ \hline 
Quantifier &74\%  &\textbf{81\%} & 77\% &\textbf{80\%}\\ \hline 
Modal &75\%	&\textbf{79\%} &76\% & \textbf{82\%} \\ \hline 
Belief &73\% &\textbf{77\%} &74\% & \textbf{78\%}\\ \hline \hline
\end{tabular}

\caption{\label{tab:error} Error analysis on MultiNLI. See  \cite{2017arXiv170708172N} for reference.}
\end{table}

\noindent \textbf{Analysis:}
How many steps it needs? We search the number of steps $t$ from 1 to 10. We observe that when $t$ increases, our model obtains a better improvement (e.g., 86.7 ($t=2$)); however when $t=5$ or $t=6$, it achieves best results (89.4) on SciTail dev set and then begins to downgrade the performance. Thus, we set $t=5$ in all our experiments.

We also looked internals of our answer module by dumping predictions of each step (the max step is set to 5). Here is an example\footnote{Its ID is id 144185n with \textbf{premise}
(And he said, What's going on?) and \textbf{hypothesis}	(I told him to mind his own business.)} from MutiNLI dev set. Our model produces total 5 labels (\textit{contradiction, neutral,	neutral, neutral, and neutral}) at each step and makes the final decision by voting \textbf{\textit{neutral}}. Surprising, we found that human annotators also gave different 5 labels: \textit{contradiction, neutral, neutral, neutral, neutral}. It shows robustness of our model which uses collective wise.

Finally, we analyze our model on the annotated subset\footnote{https://www.nyu.edu/projects/bowman/multinli/multinli\_1.0\\\_annotations.zip} of development set of MultiNLI. It contains 1,000 examples, each tagged by categories shown in Table~\ref{tab:error}. Our model outperforms the best system in RepEval 2017 \cite{2017arXiv171104289C} in most cases, except on ``Conditional" and ``Tense Difference" categories. 
We also find that SAN works extremely well on ``Active/Passive'' and ``Paraphrase'' categories. Comparing with Chen's model, the biggest improvement of SAN (50\% vs 77\% and 58\% vs 85\% on Matched and Mismatched settings respectively) is on the ``Antonym'' category.
In particular, on the most challenging ``Long Sentence" and ``Quantity/Time" categories, SAN's result is substantially better than previous systems. This demonstrates the robustness of multi-step inference.

==> Natural Language Inference/intro.tex <==
\section{Motivation}
\label{sec:mot}
The natural language inference task, also known as \textit{recognizing textual entailment} (RTE), is to infer the relation between a pair of sentences (e.g., \textit{premise} and \textit{hypothesis}).
This task is challenging, since it requires a model to fully understand the sentence meaning, (i.e., lexical and compositional semantics). For instance, the following example from MultiNLI dataset \cite{2017arXiv170405426W} illustrates the need for a form of multi-step synthesis of information between \textit{\textbf{premise}: ``If you need this book, it is probably too late unless you are about to take an SAT or GRE."}, and \textit{\textbf{hypothesis}: ``It's never too late, unless you're about to take a test."} To predict the correct relation between these two sentences, the model needs to first infer that ``\textit{SAT} or \textit{GRE}" is a ``\textit{test}", and then pick the correct relation, e.g., \textit{contradiction}. 

This kind of iterative process can be viewed as a form of multi-step inference. To best of our knowledge, all of works on NLI use a \textit{single step} inference. Inspired by the recent success of multi-step inference on Machine Reading Comprehension (MRC) \cite{hill2015goldilocks,dhingra2016gated,sordoni2016iterative,kumar15askme, liu18san, shen2017empirical,xu2018multi}, we explore the multi-step inference strategies on NLI.
Rather than directly predicting the results given the inputs, the model maintains a state and iteratively refines its predictions.
We show that our model outperforms single-step inference and further achieves the state-of-the-art on SNLI, MultiNLI, SciTail, and Quora Question Pairs datasets.

==> Natural Language Inference/model.tex <==
\section{Multi-step inference with SAN}
\label{sec:model}
\vspace{-0.1cm}
The natural language inference task as defined here involves a premise $P=\{p_0, p_1, ..., p_{m-1}\}$ of $m$ words and a hypothesis $H=\{h_0, h_1, ..., h_{n-1}\}$ of $n$ words,
and aims to find a logic relationship $R$ between $P$ and $H$, which is one of labels in a close set: \textit{entailment}, \textit{neutral} and \textit{contradiction}. 
%and aims to find a logic relationship $R$ between $P$ and $H$, which is one of labels in a close set\footnote{In SNLI, the label ``-" denotes inconsistency between annotators, and it is removed during the training and test.}: \textit{entailment}, \textit{neutral} and \textit{contradiction}. 
The goal is to learn a model $f(P, H) \rightarrow R$. 
%The training data is a set of the premise, hypothesis and relation label tuples $<P, H, R>$. 

In a single-step inference architecture, the model directly predicts $R$ given $P$ and $H$ as input. 
In our multi-step inference architecture, we additionally incorporate a recurrent state $s_t$; the model processes multiple passes through $P$ and $H$, iteratively refining the state $s_t$, before finally generating the output at step $t=T$, where $T$ is an a priori chosen limit on the number of inference steps. 
%We will now describe our model from the ground up. The main contribution of this work is the multi-step reasoning module, but in order to understand what goes into this module, we will start by describing how $P$ and $H$ are processed by the lower layers. Note the lower layers also have some novel variations that are not used in previous work. 

\begin{figure*}[h!]
\centering
\adjustbox{trim={.081\width} {.01\height} {.05\width} {.01\height},clip}%
  {\includegraphics[scale=0.6]{model_v1}}
\caption{\label{fig:model} {Architecture of the Stochastic Answer Network ({\MIN}) for Natural Language Inference.}}
\end{figure*}

Figure \ref{fig:model} describes in detail the architecture of the \textbf{s}tochastic \textbf{a}nswer \textbf{n}etwork (SAN) used in this study; this model is \textit{adapted} from the MRC multi-step inference literature \cite{liu18san}. Compared to the original SAN for MRC, in the SAN for NLI we simplify the bottom layers and % (i.e., we remove the POS tagging and NER tagging features and 
Self-attention layers since the length of the premise and hypothesis is short). We also modify the answer module from prediction a text span to an NLI classification label.  
Overall, it contains four different layers:
1) the lexicon encoding layer computes word representations; 
2) the contextual encoding layer modifies these representations in context; 
3) the memory generation layer gathers all information from the premise and hypothesis and forms a ``working memory" for the final answer module; 
4) the final answer module, a type of multi-step network, predicts the relation between the premise and hypothesis. 

%Figure \ref{fig:model} describes in detail the architecture of the \textbf{s}tochastic \textbf{a}nswer \textbf{n}etwork (SAN) we propose in this study. It contains four different layers:
%. The detailed description of each layer is introduced as follows.
%: 
%1) the lexicon encoding layer encodes different types of lexicon variants; 
%2) the contextual encoding layer attempts to capture relations between words and phrases in context; 
%3) the memory generation layer gathers all the different information from the premise and hypothesis and forms a ``working memory" for the final answer module; 
%4) the final answer module, a type of multi-step network, predicts the relation between the premise and hypothesis. 
%The detailed description of our model is provided as follows.

\noindent\textbf{Lexicon Encoding Layer}. 
%The purpose of the first layer
%This layer is to extract information from $P$ and $H$ at both the word level and character level to normalize for lexical variants.
First we concatenate word embeddings and character embeddings to handle the out-of-vocabulary words\footnote{We omit POS Tagging and Name Entity Features for simplicity}.  
Following \cite{liu18san}, we use two separate two-layer position-wise feedforward network  \cite{vaswani2017attention} to obtain the final lexicon embedings, $E^p \in \mathbb{R}^{d \times m}$ and $E^h\in \mathbb{R}^{d \times n}$, for the tokens in $P$ and $H$, respectively. Here, $d$ is the hidden size.

\noindent\textbf{Contextual Encoding Layer}. %Both premise and hypothesis use the same context encoding layer based on BiLSTM. 
Two stacked BiLSTM layers are used on the lexicon encoding layer to encode the context information for each word in both $P$ and $H$. Due to the bidirectional layer, it doubles the hidden size. We use a maxout layer \cite{goodfellow2013maxout} on the BiLSTM to shrink its output into its original hidden size. %Then, a layer normalization \cite{ba2016layer} is applied.
By a concatenation of the outputs of two BiLSTM layers, we obtain $C^p\in \mathbb{R}^{2d \times m}$ and $C^h\in \mathbb{R}^{2d \times n}$ as representation of $P$ and $H$, respectively.%, where $d$ is the hidden size of the BiLSTM. 

\noindent\textbf{Memory Layer}. We construct our working memory via an attention mechanism. 
%First, we project both $C^p$ and $C^h$ with one layer neural network $ReLU(\Theta_1 x)$ to obtain $\hat{C}^p$ and $\hat{C}^h$, respectively. Then an attention matrix $A$ is computed by using a dot-product attention:
%This is accomplished via an attention mechanism. 
First, a dot-product attention is adopted like in \cite{vaswani2017attention} to measure the similarity between the tokens in $P$ and $H$.
Instead of using a scalar to normalize the scores as in \cite{vaswani2017attention}, we use a layer projection to transform the contextual information of both $C^p$ and $C^h$:
\begin{equation}
A=dropout(f_{attention}(\hat{C}^p, \hat{C}^h)) \in \mathbb{R}^{m \times n}\\
\label{eq:align}
\end{equation}
where $A$ is an attention matrix, and dropout is applied for smoothing. 
Note that $\hat{C^p}$ and $\hat{C^h}$ is transformed from $C^p$ and $C^h$ by one layer neural network $ReLU(W_3x)$, respectively. 
Next, we gather all the information on premise and hypothesis by: $U^p = \left[C^p; C^hA\right] \in \mathbb{R}^{4d \times m}$ and $U^h = \left[C^h ; C^pA^{\prime}\right] \in \mathbb{R}^{4d \times n}$.
The semicolon $;$ indicates vector/matrix concatenation; $A^{\prime}$ is the transpose of $A$.
% by a simple concatenation of its contextual information $C^p$ and its hypothesis-aware representation $C^h \cdot A$:
% \begin{equation}
% U^p = concat(C^p, C^hA) \in \mathbb{R}^{4d \times m}
% \label{eq:gather}
% \end{equation}\vspace{-0.1cm}
% %The information of hypothesis is generated by a similar wary: 
% %The information on hypothesis is generated by a concatenation of its contextual information $C^h$ and its premise-aware representation $C^p \cdot A^{\prime}$
% \begin{equation}
% U^h = concat(C^h, C^pA^{\prime}) \in \mathbb{R}^{4d \times n}
% \label{eq:gather_h}
% \end{equation}
Last, the working memory of the premise and hypothesis is generated by using a BiLSTM based on all the information gathered: $M^p=BiLSTM([U^p; C^p])$ and $M^h=BiLSTM([U^h; C^h])$.

% \vspace{-0.2cm}
% \begin{equation}
% M^p=BiLSTM([U^p; C^p]);
% \label{eq:mem}
% \end{equation}\vspace{-0.1cm}
% %The working memory of hypothesis is generated by a BiLSTM based on the information gathered:
% \begin{equation}
% M^h=BiLSTM([U^h; C^h])
% \label{eq:mem_h}
% \end{equation}
%where the semicolon mark $;$ indicates the vector/matrix concatenation operator.

\noindent\textbf{Answer module}.
% KD: Note, I'm taking out this Chinese proverb. If used too often, I think it either reveals authorship or sounds like copying from previous papers.
%There is a Chinese proverb that says: ``wisdom of masses exceeds that of any individual."
%Unlike other multi-step inference models, which only uses a single output either at the last step, our answer module employs all the outputs of multiple step inference. Intuitively, by applying dropout, it avoids a ``step bias problem" (where models places too much emphasis one particular step's predictions) and forces the model to produce good predictions at every individual step. Further, during decoding, we reuse \textit{wisdom of masses} instead of \textit{individual} to achieve a better result.
%We call this method ``stochastic prediction dropout" because dropout is being applied to the final predictive distributions. 
Formally, our answer module will compute over $T$ memory steps and output the relation label. 
%This module is a memory network and has some similarities to other multi-step inference networks: namely, it maintains a state vector, one state per step. 
At the beginning, the initial state $s_0$ is the summary of the $M^h$: $s_0=\sum_j \alpha_j M^h_{j}$, where $\alpha_j = \frac{exp(\theta_2 \cdot M^h_j)}{\sum_{j'}exp(\theta_2 \cdot M^h_{j'})}$. At time step $t$ in the range of $\{1, 2, ..., T-1\}$, the state is defined by $s_t = GRU(s_{t-1}, x_t)$. 
Here, $x_t$ is computed from the previous state $s_{t-1}$ and memory $M^p$: $x_t=\sum_j\beta_j M^p_j$ and $\beta_j = softmax(s_{t-1}\theta_3 M^p)$. 
Following \cite{mou2015natural}, one layer classifier is used to determine the relation at each step $t \in \{0,1,\ldots,T-1\}$. 
\begin{equation}
P^r_t = softmax(\theta_4[s_t; x_t; |s_t - x_t|; s_t \cdot x_t]).
\label{eq:begin}
\end{equation}
%where the mark $;$ indicates the concatenation operator, and $j$ indicates memory index.

At last, we utilize all of the $T$ outputs by averaging the scores:
\begin{equation}
P^r = avg([P_0^{r}, P_1^{r}, ..., P_{T-1}^{r}]).
\label{eq:avg}
\end{equation}\vspace{-0.1cm}
Each $P_t^{r}$ is a probability distribution over all the relations, $\{1,\ldots,|R|\}$. %, so the average distribution is straightforward to compute.  
During training, we apply \emph{stochastic prediction dropout} before the above averaging operation. During decoding, we average all outputs to improve robustness. %The use of averaged predictions and dropout during training improves robustness. 

This stochastic prediction dropout is similar in motivation to the dropout introduced by \cite{srivastava2014dropout}. The difference is that theirs is dropout at the intermediate node-level, whereas ours is dropout at the final layer-level. Dropout at the node-level prevents correlation between features. Dropout at the final layer level, where randomness is introduced to the averaging of predictions, prevents our model from relying exclusively on a particular step to generate correct output. 
%We used a dropout rate of 0.2 in experiments. (ref 3.2)


==> Natural Language Inference/summary.tex <==
\section{Conclusion}
\label{sec:con}
We explored the use of multi-step inference in natural language inference by proposing a stochastic answer network (SAN).
Rather than directly predicting the results (e.g. relation $R$ such as entailment or not) given the input premise $P$ and hypothesis $H$, SAN maintains a state $s_t$, which it iteratively refines over multiple passes on $P$ and $H$ in order to make a prediction. 
Our state-of-the-art results on four benchmarks (SNLI, MultiNLI, SciTail, Quora Question Pairs) show the effectiveness of this multi-step inference architecture. In future, we would like to incorporate the pertrained contextual embedding, e.g., ELMo \cite{peters2018deep} and GPT \cite{radford2018improving} into our model and multi-task learning \cite{liu2019mt-dnn}.

